Evaluating Apple Intelligence's Writing Tools for Privacy Against Large Language Model-Based Inference Attacks: Insights from Early Datasets

The misuse of Large Language Models (LLMs) to infer emotions from text for malicious purposes, known as emotion inference attacks, poses a significant threat to user privacy. In this paper, we investigate the potential of Apple Intelligence's writing tools, integrated across iPhone, iPad, and MacBook, to mitigate these risks through text modifications such as rewriting and tone adjustment. By developing early novel datasets specifically for this purpose, we empirically assess how different text modifications influence LLM-based detection. This capability suggests strong potential for Apple Intelligence's writing tools as privacy-preserving mechanisms. Our findings lay the groundwork for future adaptive rewriting systems capable of dynamically neutralizing sensitive emotional content to enhance user privacy. To the best of our knowledge, this research provides the first empirical analysis of Apple Intelligence's text-modification tools within a privacy-preservation context with the broader goal of developing on-device, user-centric privacy-preserving mechanisms to protect against LLMs-based advanced inference attacks on deployed systems.

==> sec_discovery.tex <==
\section{Actionable Insights and Conclusion}

Our findings demonstrate that Apple Intelligence's on-device text modification tools significantly alter the emotional level of text, thereby affecting the ability of LLMs to accurately infer emotions. This modification serves as a foundation for an effective privacy-preserving mechanism, reducing unintentional privacy leakage in communication with LLM-based Chat bots.These results have significant implications for the system-wide integration of privacy-aware rewriting features in Natural Language Processing (NLP) systems. 

Specifically, our findings highlight the feasibility of developing on-device privacy-aware rewriting mechanisms within the ecosystem that dynamically adjust text while preserving usability. With the system-wide integration of these capabilities (in case of Apple Inc. iOS, iPadOS, and macOS), it is possible to offer customizable modification levels that balance user intention with privacy needs. For example, adaptive privacy filters could dynamically modify emotional content based on user-specific privacy levels (e.g., activating ``professional'' mode in Apple Mail, Messages or Notes when privacy is a high concern). Moreover, this research suggests that AI assistants (e.g., Siri, ChatGPT, Gemini, and CoPilot) can integrate user-configurable privacy controls that allow users to adjust how much emotion information (privacy leakage) remains in modified text. By embedding these privacy-preserving features at the system level, Apple, in particular, can further enhance its on-device AI strategy to strengthen its privacy-first policy for AI. 









==> sec_prelim.tex <==
\section{Preliminary}\label{sec:premil}
% \subsection{Related Work}

% Emotional Tone and Sentiment Detection

% \subsection{Threat Model}

%{\color{blue}Honest but curious adversary }



